Interpr\'etation de l'Arithm\'etique dans certains groupes de permutations affines par morceaux d'un intervalle

The Arithmetic is interpreted in all the groups of Richard Thompson and Graham Higman, as well as in other groups of piecewise affine permutations of an interval which generalize the groups of Thompson and Higman. In particular, the elementary theories of all these groups are undecidable. Moreover, Thompson's group $F$ and some of its generalizations interpret the Arithmetic without parameters.

==> p99.tex <==
%% format: (AMS-)LaTeX
%% project: Arithmetic in groups of permutations of an interval
%% version: Gamma (French)
%% file: part 99 (Acknowledgements)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% RECONNAISSANCES ========================================================
%: SECTION*:RECONNAISSANCES
\section*{Reconnaissances}

Les auteurs sont reconnaissants l'un l'autre.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
